VECTOR: Velocity-Enhanced GRU Neural Network for Real-Time 3D UAV Trajectory Prediction

This paper tackles the challenge of real-time 3D trajectory prediction for UAVs, which is critical for applications such as aerial surveillance and defense. Existing prediction models that rely primarily on position data struggle with accuracy, especially when UAV movements fall outside the position domain used in training. Our research identifies a gap in utilizing velocity estimates, first-order dynamics, to better capture the dynamics and enhance prediction accuracy and generalizability in any position domain. To bridge this gap, we propose a new trajectory prediction method using Gated Recurrent Units (GRUs) within sequence-based neural networks. Unlike traditional methods that rely on RNNs or transformers, this approach forecasts future velocities and positions based on historical velocity data instead of positions. This is designed to enhance prediction accuracy and scalability, overcoming challenges faced by conventional models in handling complex UAV dynamics. The methodology employs both synthetic and real-world 3D UAV trajectory data, capturing a wide range of flight patterns, speeds, and agility. Synthetic data is generated using the Gazebo simulator and PX4 Autopilot, while real-world data comes from the UZH-FPV and Mid-Air drone racing datasets. The GRU-based models significantly outperform state-of-the-art RNN approaches, with a mean square error (MSE) as low as 2 x 10^-8. Overall, our findings confirm the effectiveness of incorporating velocity data in improving the accuracy of UAV trajectory predictions across both synthetic and real-world scenarios, in and out of position data distributions. Finally, we open-source our 5000 trajectories dataset and a ROS 2 package to facilitate the integration with existing ROS-based UAV systems.

==> sections/0_abstract.tex <==
% \begin{abstract}



% This paper introduces a new prediction scheme for real-time 3D Unmanned Aerial Vehicle (UAV) trajectory using sequence-based neural networks and gated recurrent units (GRUs). Unlike existing solutions, ours combine both position and velocity historical data to attain more accurate predictions of future UAV locations. Without loss of generality, our paper focuses on an experimental setting where an UAV entity is monitored by an observer such as an interceptor drone for aerial surveillance and defense purposes. A salient feature of our research lies in the use of both synthetic and real-world 3D UAV trajectories. These trajectories, characterized by varying agility patterns, curvatures and speeds, are used to assess the performance of the proposed prediction scheme. Synthetic trajectories are simulated based on realistic configurations of the {\em Gazebo robotics simulator} and {\em PX4 Autopilot}. To assess the suitability of our prediction algorithm, real-world drone trajectories are considered including the {\em UZH-FPV} and {\em Mid-Air} drone racing datasets. To enhance the memory capabilities of the prediction process, sequence-based neural networks are considered. GRU cells encode the prediction memory and the hidden/latent states. Training data consisting of drone 3D position and velocity samples are used to train the GRU-based prediction algorithm. The reported results indicate the superiority of the velocity-based position prediction algorithm. Additionally, our algorithm outperforms existing ones based on recurrent neural networks (RNNs). On equal footing based on dataset size, our GRU-based model outperforms those using transformers, as the latter suffer from the scaling problem. 24 different model configurations are assessed against simulated and real-world data achieving average mean square error (MSE) ranging from $2 \times 10^{-8}$ to $2 \times 10^{-7}$. Finally, the superiority of velocity-based predictions is confirmed in all  reported experiments.
% \end{abstract}



%
%- **Limitations**: these comments are worth considering to improve the abstract 
% What is the problem statement, and what is the gap addressed in the literature?
%- The study focuses on comparing GRU models, but it does not mention if other types of models like LSTM or transformer-based models were considered. This may limit the comprehensiveness of the study's findings.
%- The abstract does not clearly explain the novelty of the proposed approach compared to existing methods. The comparison is limited to 24 GRU models only.
%- It is unclear how the accuracy and generalizability of the models were measured and what specific metrics were used.
%- The abstract does not mention any possible limitations or drawbacks of the proposed method, which could indicate a lack of rigorous evaluation.
%- The abstract does not provide a clear implication of the results or its potential applications in real-world scenarios.
%- **Proposed Title**: "Real-Time 3D UAV Trajectory Prediction Using Gated Recurrent Neural Networks: A Comparative Study with Synthetic and Real-World Datasets"
%The authors analyze the influence of dataset diversity on model performance without clearly defining what constitutes 'dataset diversity.' More clarity on this aspect is needed to understand the methodology better.
%The paper reports that velocity-based trajectories are more generalized and robust than position prediction. However, it does not provide an in-depth explanation or supporting evidence as to why this is the case. Further exploration in this area could strengthen the paper's argument and provide more insights into the effectiveness of velocity-based trajectories.

% \begin{abstract}

% This paper introduces a new prediction scheme for real-time 3D Unmanned Aerial Vehicle (UAV) trajectory using sequence-based neural networks and gated recurrent units (GRUs). Unlike existing solutions, ours combines both position and velocity historical data to attain more accurate predictions of future UAV locations. Without loss of generality, our paper focuses on an experimental setting where a UAV entity is monitored by an observer, such as an interceptor drone, for aerial surveillance and defense purposes. A salient feature of our research lies in the use of both synthetic and real-world 3D UAV trajectories. These trajectories, characterized by varying agility patterns, curvatures, and speeds, are used to assess the performance of the proposed prediction scheme. Synthetic trajectories are simulated based on realistic configurations of the {\em Gazebo robotics simulator} and {\em PX4 Autopilot}. To further validate the robustness of our approach, we conducted real-world experiments using a quadcopter following arbitrary flight patterns, demonstrating the practical applicability of the prediction models. In addition, real-world drone trajectories were considered, including the {\em UZH-FPV} and {\em Mid-Air} drone racing datasets. To enhance the memory capabilities of the prediction process, sequence-based neural networks are employed, with GRU cells encoding the prediction memory and hidden/latent states. Training data consisting of drone 3D position and velocity samples are used to train the GRU-based prediction algorithm. Results show that GRU-based models, particularly those utilizing velocity data, outperform existing methods, including RNNs and LSTMs, across 24 model configurations. In real-world experiments, velocity-based predictions demonstrated superior accuracy, achieving an average mean square error (MSE) between $2 \times 10^{-8}$ to $2 \times 10^{-7}$, validating the robustness of the approach across diverse scenarios.




% \end{abstract}

% Proposed by Prof. Anis

\begin{abstract}
This paper addresses the challenge of predicting 3D trajectories for Unmanned Aerial Vehicles (UAVs) in real-time, a critical task for applications like aerial surveillance and defense. Current prediction models primarily leverage only position data, which may not provide the most accurate forecasts for UAV movements and usually fail outside the position domain used in the training phase. Our research identifies a gap in utilizing velocity estimates, first-order dynamics, to better capture the dynamics and enhance prediction accuracy and generalizability in any position domain.
To bridge this gap, we introduce a trajectory prediction scheme, using sequence-based neural networks with Gated Recurrent Units (GRUs), to forecast future velocity and positions based on velocity historical estimates instead of position measurements. This approach is designed to improve the predictive capabilities over traditional methods that rely solely on recurrent neural networks (RNNs) or transformers, which can struggle with scalability in this context.
Our methodology employs both synthetic and real-world 3D UAV trajectory data, incorporating diverse patterns of agility, curvature, and speed. Synthetic data is generated using the Gazebo robotics simulator and PX4 Autopilot, while real-world data is sourced from the UZH-FPV and Mid-Air drone racing datasets. We train the GRU-based models on drone 3D position and velocity samples to capture the dynamics of UAV movements effectively.
Quantitatively, the proposed GRU-based prediction algorithm demonstrates superior performance, achieving a mean square error (MSE) ranging from $2 \times 10^{-8}$ to $2 \times 10^{-7}$. This performance outstrips existing state-of-the-art RNN models. Overall, our findings confirm the effectiveness of incorporating velocity data in improving the accuracy of UAV trajectory predictions across both synthetic and real-world scenarios, in and out of position data distributions. Finally, we open-source our 5000 trajectories dataset and a ROS 2 package to facilitate the integration with existing ROS-based UAV systems.
\end{abstract}

==> sections/name.tex <==
This study implemented the experimental framework to evaluate the efficacy of Gated Recurrent Unit (GRU) models in predicting drone trajectories for both position and velocity segments. Our experimental framework provides a comprehensive dataset preparation, model architecture, training procedures, and evaluation metrics, focusing on the model's performance under various conditions, including model complexity and normalization steps.

\subsection*{A. Experimental Design}
\subsubsection*{Variables}
\begin{itemize}
    \item \textbf{Independent Variables:} Model complexity (64x2, 128x3, 256x5 hidden units x layers), normalization methods (Max Norm, Whitening).
    \item \textbf{Dependent Variable:} Prediction accuracy (MSE, RMSE, MAE, R-squared).
\end{itemize}

\subsubsection*{Model Architecture}
The model architecture and configuration used in this experiment are primarily focused on investigating the model complexity and how it might affect the GRU-based Trajectory Predictor's performance. The architecture of the GRU model is pivotal in understanding different patterns and trends of drone trajectory prediction. The Trajectory Predictor, as shown in Figure /ref{fig1}, implemented in PyTorch, comprises an encoder-decoder structure using GRU layers and a fully connected output layer, providing a robust framework for capturing the temporal dynamics of trajectories.

The model's encoder uses a GRU layer incorporating dropout regularization to reduce overfitting. The decoder, an additional GRU layer, reconstructs the trajectory output. A fully connected layer then converts the decoder output into the final projected trajectory. Thanks to its architecture, the model can efficiently learn complex temporal patterns from drone flying data.

\subsubsection*{Data Sets}
The models are trained and tested on integrated and simulation-only datasets. The integrated dataset comprises short and long historical 3d UAV trajectories and 5000 real-time drone trajectories. As explained in section II, the simulation-only dataset includes only the 5000 real-time trajectories. 

\subsection*{B. Procedure}
\subsubsection*{Model Training}

The training procedure has involved a variety of the model's complexity by adjusting the hidden dimension and layer count configurations and keeping the input (3D coordinates) and output dimensions constant. In particular, we looked into three setups, including the default design consisting of 64 hidden units with two layers, which provides a good compromise between computational performance and model complexity. Then, we considered 128 three-layered hidden units with more intricate models, which might anticipate extracting more minute information from the data and enhancing predictions but come at the expense of additional processing power. After that, a model with five layers and 256 hidden units is the most complicated model in our analysis. It was created to see how well our architecture could handle the mix and simulation-only dataset. Other parameters, such as the learning rate set to 0.001 with a dropout rate of 0.5, were maintained constant throughout these studies. The Adam optimizer optimized the models \cite{kingma2014adam}, trained with the Mean Squared Error Loss function, and controlled by a learning rate scheduler with a gamma of 0.1 and a step size of 50.

Our approach systematically alters the model's complexity to find the best compromise between computational efficiency and accuracy. With the help of this method, we can comprehend how the GRU network's width and depth affect the model's capacity to forecast drone trajectories in various scenarios.

In the training phase, the integrated and simulation-only datasets were used to train the GRU model across many epochs, precisely set at 1000. However, we put an early stopping mechanism in place to avoid over-training by the models and maximize training time. With this strategy, the model stops training when the validation loss stops improving. This will help you prevent overfitting and pointless calculations. A patience parameter of 100 epochs was used to control this further to establish the early stopping threshold. This indicates that the training process is stopped if the validation loss does not go down for 100 consecutive epochs. This is also important to guarantee that the saved model performed the best on the validation set, as shown by the lowest validation loss.

Regarding the loss function, we employed the Mean Squared Error (MSE) Loss, and it is mathematically represented as \ref{eq8}:

\begin{equation}
    \text{MSE Loss} = \frac{1}{n} \sum_{i=1}^{n} (y_i - \hat{y}_i)^2
\label{eq8}
\end{equation}

\noindent where $y_i$ is the actual value, $\hat{y}_i)$ is the predicted value, and n is the number of samples. This loss function is particularly suited for our task as it effectively captures the average squared difference between the predicted and actual trajectory points, emphasizing more significant errors.

The loss is reduced by adjusting the model's parameters through the optimizer by making forward and backward passes through the model as part of the training loop for every batch of the training data. Therefore, the Adam optimizer was employed due to its adeptness in managing sparse gradients and its capacity for adaptive learning rate. In order to improve the model's convergence, a learning rate scheduler was also used to modify the learning rate during training.

We concentrated on the model set with 128 hidden units as an extension of our training and hyperparameter tuning approach, investigating the tradeoff between performance and growing model complexity. For this analysis, the model's layer count was varied from two to ten. This investigation aimed to determine how the GRU network's capacity to learn and predict drone trajectories is impacted by its depth.

The 128 hidden unit configuration was chosen for this analysis due to its intermediate position between the most sophisticated model and the baseline. Therefore, we consider using this configuration for studying the consequences of growing complexity without going to the limits of the computing power of the largest model configuration. We observed changes in the model's learning dynamics and validation set performance by progressively increasing the number of layers. We could establish a direct correlation between model complexity and performance through hyperparameter optimization. 

\subsubsection*{Model Evaluation}
The model's performance is assessed using MSE, RMSE, MAE, and R-squared across different complexities and normalization methods.

\subsection*{C. Analysis}
\subsubsection*{Statistical Analysis}
The experiment employs ANOVA to analyze the effects of independent variables on prediction accuracy and explores interaction effects between model complexity and normalization methods.

\subsubsection*{Performance Evaluation}

We evaluated the performance of our GRU-based trajectory predictor model in our study using an extensive set of evaluation metrics. These measurements are essential to comprehend in-depth how well the model predicts drone trajectories. Each metric provides a different viewpoint on the accuracy and generalization capacity of the model.

\subsubsection{Mean Squared Error (MSE):}
The MSE is a standard metric for regression tasks, measuring the average of the squares of the errors. It is calculated as in equation \ref{eq8}

\begin{equation}
    \text{MSE} = \frac{1}{n} \sum_{i=1}^{n} (y_i - \hat{y}_i)^2
\label{eq9}
\end{equation}

\subsubsection{Root Mean Squared Error (RMSE):}
RMSE provides a more interpretable version of MSE by taking the square root of the MSE. It is defined as in \ref{eq10}:

\begin{equation}
    \text{RMSE} = \sqrt{\frac{1}{n} \sum_{i=1}^{n} (y_i - \hat{y}_i)^2}
\label{eq10}
\end{equation}

\subsubsection{Mean Absolute Error (MAE):}
MAE measures the average magnitude of the errors in a set of predictions without considering their direction. It is given by equation \ref{eq11}:

\begin{equation}
    \text{MAE} = \frac{1}{n} \sum_{i=1}^{n} |y_i - \hat{y}_i|
\label{eq11}
\end{equation}

\subsubsection{R-squared (Coefficient of Determination):}

R-squared is a statistical measure representing the proportion of the variance for the dependent variable explained by the independent variables. It is expressed as \ref{eq12}:

\begin{equation}
    R^2 = 1 - \frac{\sum_{i=1}^{n} (y_i - \hat{y}_i)^2}{\sum_{i=1}^{n} (y_i - \overline{y})^2}
\label{eq12}
\end{equation}

\noindent where, $\overline{y}$ is the mean of the true values.

Collectively, these metrics provide a robust framework for evaluating the model's predictive performance, allowing us to assess its accuracy, error magnitude, and the proportion of variance explained by the model, which is crucial for developing effective trajectory prediction models.



